Copula Geometry and Second-Order Calibration of Heavily Right Aggregation

Heavy-tailed $p$-value combination tests are attractive under unknown dependence because their null tails can be first-order robust even when the exact dependent null distribution is unavailable. That robustness does not resolve calibration: $\Pr\{T>q(\alpha)\}=\alpha+o(\alpha)$ neither quantifies the remaining size error nor determines its sign. We develop a second-order calibration theory for positive Half-Cauchy and reciprocal, or harmonic-mean, aggregation. After exact marginal standardization, extremal dependence is represented by an index-one exponent measure on the coordinate-face lattice. Its support separates axial, full-interior, proper-face, and mixed geometries. A M\"obius decomposition shows how the noncompact weighted half-space probes every face, while quantitative face limits determine whether the correction is integrable, critically amplified, or nonintegrable. With common-factor inversion and a tail-to-calibration map, this yields machinery applicable beyond individual parametric copula families. The results include an integrable hidden-face transfer theorem, a sharp fixed-dimensional local-corner theorem with explicit higher-face control, a common-heavy-factor theorem, and size and critical-value expansions relative to independence. Gaussian, standard multivariate-$t$, positive Clayton, and max-linear pair-shock models exhibit distinct power, logarithmic, radial--angular, and proper-face mechanisms; the Gaussian weighted-half-space transfer is conditional on explicit face-boundary hypotheses. Thus dependence geometry determines the rate, coefficient, and direction of the calibration error left unresolved by first-order validity. Asymptotics use $t\to\infty$, equivalently vanishing significance levels.

==> copula-geometry-second-order-preamble.tex <==
% Shared packages, theorem declarations, and notation for all builds.
\ifdefined\CGSOAOS
  \RequirePackage{amsmath,amssymb,amsthm,mathtools}
  \RequirePackage[numbers]{natbib}
\else
  \usepackage[margin=1in]{geometry}
  \usepackage{amsmath,amssymb,amsthm,mathtools}
  \usepackage[T1]{fontenc}
  \usepackage{newtxtext,newtxmath}
\fi

\usepackage{booktabs}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{longtable}
\ifdefined\CGSOAOS
  \RequirePackage{etoolbox}
  % Compact tables only in the AoS builds.  The arXiv layout is unchanged.
  \AtBeginEnvironment{longtable}{%
    \scriptsize
    \setlength{\tabcolsep}{2pt}%
    \renewcommand{\arraystretch}{0.88}%
  }
  \AtBeginEnvironment{tabular}{%
    \scriptsize
    \setlength{\tabcolsep}{2pt}%
    \renewcommand{\arraystretch}{0.88}%
  }
\fi
\ifdefined\CGSOAOS
  \ifdefined\CGSOSUPPLEMENT
    \usepackage{pdflscape}
  \fi
\else
  \usepackage{pdflscape}
\fi
\usepackage{aliascnt}
\ifdefined\CGSOAOS\else
  \usepackage{xr-hyper}
\fi
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage[nameinlink,capitalize]{cleveref}

\ifdefined\CGSOAOS
  \startlocaldefs
\fi

\numberwithin{equation}{section}

\ifdefined\CGSOAOS
  \theoremstyle{plain}
\else
  \newtheoremstyle{thmstyleone}
    {\topsep}{\topsep}{\itshape}{}{\bfseries}{.}{5pt plus 1pt minus 1pt}{}
  \newtheoremstyle{thmstyletwo}
    {\topsep}{\topsep}{\normalfont}{}{\bfseries}{.}{5pt plus 1pt minus 1pt}{}
  \theoremstyle{thmstyleone}
\fi

\newtheorem{theorem}{Theorem}[section]
\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\ifdefined\CGSOAOS\else
  \newaliascnt{definition}{theorem}
  \newtheorem{definition}[definition]{Definition}
  \aliascntresetthe{definition}
\fi
\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\newaliascnt{conjecture}{theorem}
\newtheorem{conjecture}[conjecture]{Conjecture}
\aliascntresetthe{conjecture}
\newaliascnt{openproblem}{theorem}
\newtheorem{openproblem}[openproblem]{Open problem}
\aliascntresetthe{openproblem}

\ifdefined\CGSOAOS
  \theoremstyle{definition}
  \newaliascnt{definition}{theorem}
  \newtheorem{definition}[definition]{Definition}
  \aliascntresetthe{definition}
\else
  \theoremstyle{thmstyletwo}
\fi
\newaliascnt{example}{theorem}
\newtheorem{example}[example]{Example}
\aliascntresetthe{example}
\newtheorem*{remark}{Remark}
\newtheorem*{claim}{Claim}

% Fallback dictionary for PDF bookmarks.
\providecommand{\sectionautorefname}{Section}
\providecommand{\theoremautorefname}{Theorem}
\providecommand{\propositionautorefname}{Proposition}
\providecommand{\lemmaautorefname}{Lemma}
\providecommand{\definitionautorefname}{Definition}
\providecommand{\corollaryautorefname}{Corollary}
\providecommand{\conjectureautorefname}{Conjecture}
\providecommand{\openproblemautorefname}{Open problem}
\providecommand{\exampleautorefname}{Example}

% Swap \cref to \autoref strictly inside PDF bookmark strings.
\pdfstringdefDisableCommands{%
  \let\cref\autoref
}

% Once appendix numbering begins, all three heading levels use the common
% cleveref type ``appendix'': Appendix A, Appendix A.1, Appendix A.1.1.
\newcommand{\AppendixCrefSetup}{%
  \crefname{appendix}{Appendix}{Appendices}%
  \crefalias{section}{appendix}%
  \crefalias{subsection}{appendix}%
  \crefalias{subsubsection}{appendix}%
}

\newcommand{\R}{\mathbb R}
\newcommand{\Pp}{\mathbb P}
\newcommand{\E}{\mathbb E}
\newcommand{\bH}{\boldsymbol H}
\newcommand{\bY}{\boldsymbol Y}
\newcommand{\bU}{\boldsymbol U}
\newcommand{\bw}{\boldsymbol w}
\newcommand{\bx}{\boldsymbol x}
\newcommand{\bs}{\boldsymbol s}
\newcommand{\HCCT}{T_{\mathrm{HCCT}}}
\newcommand{\FHCw}{F_{\mathrm{HC},\boldsymbol w}}
\newcommand{\FRw}{F_{\mathrm{R},\boldsymbol w}}
\newcommand{\MRV}{\mathrm{MRV}}

\newcommand{\papertitle}{Copula Geometry and Second-Order Calibration of Heavily Right Aggregation}
\newcommand{\paperdisplaytitle}{Copula Geometry and Second-Order Calibration of\\Heavily Right Aggregation}
\newcommand{\paperruntitle}{Copula Geometry and Second-Order Calibration}
\newcommand{\authoraffiliation}{Department of Statistics and Operations Research, University of North Carolina at Chapel Hill}
\newcommand{\authoremail}{tianletl@unc.edu}
\newcommand{\paperdate}{August 27, 2026}

\ifdefined\CGSOAOS
  \newcommand{\ProofLocation}{the Supplementary Material}
  \newcommand{\FullLedgerLabel}{the Supplementary Material}
  \newcommand{\FullLedgerAppendix}{the Supplementary Material}
  \newcommand{\FullLedgerPlacement}{the Supplementary Material}
  \newcommand{\CounterTailSource}{the Supplementary Material}
  \newcommand{\TechnicalLocation}{the Supplementary Material}
  \newcommand{\LiteratureAuditLocation}{Appendix~C of the Supplementary
    Material~\cite{LiuSupplement2026}}
  \newcommand{\GeometryFigureWidth}{0.90\textwidth}
\else
  \newcommand{\ProofLocation}{\cref{app:proofs}}
  \newcommand{\FullLedgerLabel}{\cref{tab:copula-hierarchy}}
  \newcommand{\FullLedgerAppendix}{\cref{app:copula-classification-proofs}}
  \newcommand{\FullLedgerPlacement}{\cref{tab:copula-hierarchy} in
    \cref{app:copula-classification-proofs}}
  \newcommand{\CounterTailSource}{\cref{eq:appendix-counter-tail}}
  \newcommand{\TechnicalLocation}{\cref{app:technical-extensions}}
  \newcommand{\LiteratureAuditLocation}{\cref{sec:story}}
  \newcommand{\GeometryFigureWidth}{\textwidth}
  \emergencystretch=2em
\fi

\ifdefined\CGSOAOS
  \endlocaldefs
\fi

